Review of Neutron Yield from (${\alpha}$, n) Reactions: Data, Methods, and Prospects

Understanding the radiogenic neutron production rate through the (${\alpha}$, n) reaction is crucial in many areas of physics, including dark matter searches, neutrino studies, and nuclear astrophysics. In addition to its relevance for fundamental research, the (${\alpha}$, n) reaction also plays a significant role in nuclear energy technologies, for example by contributing to neutron production in subcritical systems using UO$_{2}$, as well as in applications such as medical physics. This review examines the current state of (${\alpha}$, n) yield calculations and neutron spectra, describes the computational tools used for their estimation, and discusses the available cross-section data. We explore the uncertainties affecting (${\alpha}$, n) yield estimations and propose a strategy to enhance their accuracy. Furthermore, this paper discusses and emphasizes the need for new measurements of (${\alpha}$, n) cross-sections for a variety of relevant materials. Such measurements are essential for improving neutron flux predictions, which are crucial for reducing uncertainties in sensitivity estimates for next-generation physics experiments operating in the keV--MeV range.

==> TexFiles/Data.old.tex <==
\section{Cross sections}
\label{sec:Xsec:}


\textbf {Contributors: Vitaly, Shawn, Maxim, Valentina, Susana, Roberto.....} \\

%{\color{red} VK: Do we want to include a couple of figures here, for instance cross-section (for a couple of isotopes as a function of alpha energy from various measurements and models?}

\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.25\linewidth]{./Plots/C13_a-n_xs}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.25\linewidth]{./Plots/C13_a-n_xs_logy}
\end{subfigure}
\caption{$^{13}$C\alphan$^{16}$O cross section as a function of energy.}
\label{fig:figC}
\end{figure}

\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.25\linewidth]{./Plots/F19_a-n_xs}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.25\linewidth]{./Plots/F19_a-n_xs_logy}
\end{subfigure}
\caption{$^{19}$F\alphan$^{22}$Na cross section as a function of energy.}
\label{fig:figF}
\end{figure}

\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.25\linewidth]{./Plots/B10_a-n_xs}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.25\linewidth]{./Plots/B10_a-n_xs_logy}
\end{subfigure}
\caption{$^{10}$B\alphan$^{13}$N cross section as a function of energy.}
\label{fig:figB}
\end{figure}

\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.25\linewidth]{./Plots/Ar40_a-n_xs}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=1.25\linewidth]{./Plots/Ar40_a-n_xs_logy}
\end{subfigure}
\caption{$^{40}$Ar\alphan$^{43}$Ca cross section as a function of energy.}
\label{fig:figAr}
\end{figure}


The energy dependent cross-sections of \alphan\ reactions are isotope-dependent and can be calculated using nuclear physics codes, such as \EMPIRE\footnote{Currently in version 3.2 available at \url{https://www-nds.iaea.org/empire/}.}~\cite{Herman2007,Herman2015} or \TALYS\footnote{Currently in version 1.96 available at \url{https://www-nds.iaea.org/talys/}.}~\cite{Koning2012,Koning2021}, or taken from experimental data where available. They can also be taken from available libraries, either evaluated like \JENDL~\cite{Iwamoto_jendl-5:2023} or produced using the toolkits as above, like \TENDL~\cite{koning_tendl_2019} containing a library of cross-sections from the TALYS code. The energy threshold of these reactions is determined by the $Q$-value of the reaction and the Coulomb barrier that suppresses the reaction probability even if the $\alpha$-particle energy is above the threshold determined by the $Q$-value. Hence, the \alphan\ reactions are important for low- and medium-$Z$ nuclei while the neutron yield per unit concentration of a radioactive isotope from elements heavier than copper is quite small. Figures \ref{fig:figC} to \ref{fig:figAr} show a comparison of cross section data taken from different sources for different target nuclei.

\subsection{Databases}
\label{sec:Xsec:DB}

The Experimental Nuclear Reaction Data (\EXFOR) library \cite{otuka_towards_2014} (\CSISRS\ in USA) contains an extensive compilation of experimental nuclear reaction data, based on numerical data sets and bibliographical information of \num{22000} experiments since the beginning of nuclear science and it is updated monthly. The associated online database retrieval system provides access to data (by selecting target, reaction, quantity or energy range) and different tools for plotting and data comparison. It is publicly available at the websites of the International Atomic Energy Agency Nuclear Data Section\footnote{\url{http://www-nds.iaea.org/exfor}}, the U.S. National Nuclear Data Center\footnote{\url{http://www.nndc.bnl.gov/exfor}} and several mirrors. The energy dependent experimental \alphan\ cross section data available in the \EXFOR\ database for a particular target isotope are limited and often not available for the full energy range. It is possible that multiple measurements of the same isotope often disagree with each other. Furthermore, measurements catalogued by EXFOR often have inconsistent treatments of experimental uncertainties, often accounting for varying levels of precision.

On the other hand, only two sets of evaluated \alphan\ cross section data libraries are available.

\JENDL\ (Japanese Evaluated Nuclear Data Library) \cite{Iwamoto_jendl-5:2023} provides a library of reaction data for various application fields (the so-called ``general purpose files'') and a set of extra libraries for some particular application field (the so-called ``special purpose files'')\footnote{\url{https://wwwndc.jaea.go.jp/jendl/jendl.html}}. The last release of the main library was in 2021 and it got the name \JENDLv{5}. Among others it includes information for 795 nuclides for neutron-induced reactions and 18 nuclides for alpha-induced reactions in the energy range up to \SI{200}{\MeV} and \SI{15}{\MeV}, respectively.
%\footnote{\url{https://wwwndc.jaea.go.jp/jendl/j5/j5.html}}
%{\color{red} MP: latest release is JENDL-5 (2021) - 795 nuclides for neutron-induced reactions and 18 nuclides for alpha-induced reactions}. 
These 18 nuclides are important mainly in nuclear fuel-cycle applications. They are \ce{^6Li}, \ce{^7Li}, \ce{^9Be}, \ce{^10B}, \ce{^11B}, \ce{^12C}, \ce{^13C}, \ce{^14N}, \ce{^15N}, \ce{^17O}, \ce{^18O}, \ce{^19F}, \ce{^23Na}, \ce{^27Al}, \ce{^28Si}, \ce{^29Si} and \ce{^30Si}. The alpha-particle sublibrary includes neutron production cross sections, outgoing neutron energy and angular distribution data.
\JENDL\ is a truly evaluated library providing recommended nuclear data. Cross sections in the JENDL library are typically derived from the measurements also included in EXFOR, with adjustments made to account for disagreements between different measurements and nuclear model codes (mainly using the \mEXIFON\ and \EGNASH\ codes) used to aid the extrapolation of these data.  In some cases, the total neutron production cross section is  adjusted to reproduce measured thick-target neutron yields. All data in \ENDFv{6} format can be retrieved from the dedicated page on the web-site of the JAEA Nuclear Data Center.
%\footnote{\url{https://wwwndc.jaea.go.jp/ftpnd/jendl/jendl-5-a.html}}

\TENDL\ (\TALYS-based Evaluated Nuclear Data Library) \cite{koning_tendl_2019} is a major nuclear data library which provides the output of the \TALYS\ nuclear model code system for direct use in both basic physics and applications. \TENDL\ contains evaluations for seven types of incident particles (neutrons, protons, deuterons, tritons, \ce{^3He}, $\alpha$-particles, and \grs), for about \num{2800} isotopes and up to energies of \SI{200}{\MeV} for some cases. The 11$^{th}$ version is \TENDLv{2021}, based on both default and adjusted \TALYS\ calculations and data from other sources. First release was in 2008 and the latest ones are \TENDLv{2015}, \TENDLv{2017}, \TENDLv{2019} and \TENDLv{2021}. Since 2015, \TENDL\ is mainly developed at PSI and the IAEA (Nuclear Data Section). Data files are openly available\footnote{\url{https://tendl.web.psi.ch/tendl_2021/talys.html}}. In the alpha sub-library, tabulated data for total and partial cross section data and spectra for virtually all isotopes can be found, including the \alphanx\ process; energy is given in \si{\MeV} and cross section in \si{\milli\barn}. Evaluated formatted data (\ENDF) are also available. Both total non-elastic cross section and cross sections for explicit reaction channels are provided, although some problems are reported for the latter in~\cite{mendoza_neutron_2020} for a number of isotopes.


\begin{table}[htb]
    \renewcommand{\arraystretch}{1.31}
    \centering
    \caption{Isotopes for which \alphan\ cross sections are catalogued in the EXFOR and JENDL databases.}
    \begin{tabular}{ccc||ccc||ccc}\hline\hline 
        Isotope    & EXFOR & JENDL & Isotope    & EXFOR & JENDL & Isotope    & EXFOR & JENDL \\\hline\hline
        \ce{^6Li}  & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   & 
        \ce{^7Li}  & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   & 
        \ce{^8Li}  & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^9Be}  & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   & 
        \ce{^10B}  & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   & 
        \ce{^11B}  & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   \\
        \ce{^12C}  & \textcolor{Red}{No}    & \textcolor{Blue}{Yes}   & 
        \ce{^13C}  & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   & 
        \ce{^14N}  & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   \\
        \ce{^15N}  & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   & 
        \ce{^16O}  & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^17O}  & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   \\
        \ce{^18O}  & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   & 
        \ce{^19F}  & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   & 
        \ce{^20Ne} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^21Ne} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^22Ne} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^23Na} & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   \\ 
        \ce{^24Mg} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^25Mg} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^26Mg} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^27Al} & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   & 
        \ce{^28Si} & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   & 
        \ce{^29Si} & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   \\
        \ce{^30Si} & \textcolor{Blue}{Yes}   & \textcolor{Blue}{Yes}   & 
        \ce{^31P}  & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^34S}  & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^35Cl} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^41K}  & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^40Ca} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^48Ca} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^45Sc} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^46Ti} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\  
        \ce{^48Ti} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^51V}  & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^50Cr} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^55Mn} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^54Fe} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^59Co} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^58Ni} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^60Ni} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^62Ni} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^64Ni} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^63Cu} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^65Cu} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^64Zn} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^66Zn} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^68Zn} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^70Zn} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^69Ga} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^71Ga} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^70Ge} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^72Ge} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^74Ge} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^76Ge} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^75As} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^76Se} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^86Sr} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^89Y}  & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^93Nb} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^92Mo} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^94Mo} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^100Mo}& \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^98Ru} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^107Ag}& \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^109Ag}& \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^115In}& \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^121Sb}& \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^123Sb}& \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \ce{^130Te}& \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^127I} & \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    & 
        \ce{^131Ta}& \textcolor{Blue}{Yes}   & \textcolor{Red}{No}    \\
        \hline\hline 
    \end{tabular}
    \label{tab:xsdata}
\end{table}





\begin{table}[htb]
    \centering
    \renewcommand{\arraystretch}{1.31}
    \caption{Naturally occurring isotopes for which there are currently no measured \alphan\ cross sections in the \SIrange{4}{10}{\MeV} energy range catalogued in EXFOR. Elements for which * is listed for the mass number have no data available for any of their naturally occurring isotopes. In addition to the isotopes listed below, data are lacking for all elements with atomic numbers greater than that of iodine, with the exception of \ce{^131Ta}. Red elements (all except \ce{Ni} and \ce{V}) are those for which missing isotopes constitute an $\mathcal{O}(1)$ contribution to the element's total neutron yield at natural abundance, relative to the dominant contributor.}
    \begin{tabular}{rrrrrrr}\hline\hline 
        {\color{red} \ce{^{32,33,36}S}} & {\color{red} \ce{^37Cl}} & {\color{red} \ce{^*Ar}} & {\color{red} \ce{^{39,40}K}} & {\color{red} \ce{^{42-44,46}Ca}} & {\color{red} \ce{^{47,49,50}Ti}} & \ce{^50V} \\
        {\color{red} \ce{^{52-54}Cr}} & {\color{red} \ce{^{56-58}Fe}} & \ce{^{61}Ni} & {\color{red} \ce{^67Zn}} & {\color{red} \ce{^73Ge}} & {\color{red} \ce{^{74,77,78,80,82}Se}} & {\color{red} \ce{^{*}Br}} \\
        {\color{red} \ce{^*Kr}} & {\color{red} \ce{^*Rb}} & {\color{red} \ce{^{84,87,88}Sr}} & {\color{red} \ce{^*Zr}} & {\color{red} \ce{^{95,96-98}Mo}} & {\color{red} \ce{^{96,99-102,104}Ru}} & {\color{red} \ce{^*Rh}} \\
        {\color{red} \ce{^*Pd}} & {\color{red} \ce{^*Cd}} & {\color{red} \ce{^113In}} & {\color{red} \ce{^*Sn}} & {\color{red} \ce{^{120,122-126,128}Te}} & \\
        \hline\hline 
    \end{tabular}
    \label{tab:missing_xsdata}
\end{table}

Isotopes for which there exist experimentally measured and evaluated cross sections that overlap with the energy range of interest are summarized in Tab.~\ref{tab:xsdata}. While the available data cover most naturally occurring isotopes, several lack data, many of which may by important for low-background experiments. 
These isotopes are summarized in Tab.~\ref{tab:missing_xsdata}.
Elements for which the missing isotopes constitute an $\mathcal{O}(1)$ contribution to the total neutron yield relative to the dominant contributor are colored red, as computed by \NeuCBOT\ for \SI{10}{\MeV} $\alpha$-particles, using cross sections computed by TALYS. 
In addition to the isotopes explicitly listed in this table, cross section measurements do not exist for all other isotopes with atomic numbers greater than that of iodine, with the exception of $^{131}$Ta. However, we note that the total neutron yield of such heavy isotopes tends to be low: for example, \NeuCBOT\ predicts an \alphan\ yield of $6.9\times10^{-10}$ $n/\alpha$ at \SI{10}{MeV}. \textcolor{purple}{Maxim: For which isotope is this number given?}
 
Elements that are lacking \alphan\ cross section measurements are typically in the mid-$Z$ range, including metals and noble gases, along with other elements that are commonly used in detector structural materials or as targets for low-background experiments. 

A detailed comparison of the results from \JENDLan\ and \TENDLv{2014}, \TENDLv{2015}, and \TENDLv{2017} is done in~\cite{mendoza_neutron_2020}; \TENDL\ is found to provide larger neutron production cross sections in most of the cases, with a few exceptions.

\subsection{Models}
\label{sec:Xsec:Models}
Leading Editor: \underline{Maxim.}, Vicente \\

% Holger 2023-06-27: move introductionary parts from §VI.D to here and merge it with the existing text
Depending on the kinetic energy $E_\mathrm{\alpha}$ of the incident $\upalpha$ particle, various reactions can occur\footnote{See e.g.\ \cite{Bertulani2019} for an introduction into nuclear reaction theory.}: below the Coulomb barrier of the target nucleus $X$, the incident particle may scatter elastically $\mathrm{X(\alpha, \alpha)X}$, at higher energies, inelastic scattering $\mathrm{X(\alpha, \alpha')X}^*$ may leave the target nucleus $X$ in an excited level. At low energies and especially for deformed nuclei this may be a collective excitation e.g.\ rotation or vibration. At higher energies, stripping reactions may cause a neutron emission. Above the Coulomb barrier, the incident $\upalpha$ can be captured: after a pre-equilibrium phase the incident nucleons are thermalized, resulting in the creation of a compound nucleus ${}^{A+2}_{Z+2}X^*$ excited by the added energy: both the kinetic energy of the $\upalpha$ and the binding energy $S_\mathrm{\alpha}$. The compound nucleus may de-excite via several decay channels: e.g.\ either via $\upgamma$ transition to the ground state or, if the incident energy $E_\mathrm{\alpha}+S_\mathrm{\alpha}$ is a multiple of the neutron separation energy $S_\mathrm{n}$, via the emission of one or more neutrons together with one or more $\upgamma$ particles, i.e. \alphan, ($\alpha$, $n \gamma$), ($\alpha$, 2$n \gamma$), ($\alpha$, $2n 2\gamma$), \ldots, ($\alpha$, $x n y \gamma$) with the related exclusive excitation functions $\sigma_{\mathrm{\alpha},x \mathrm{n} y \mathrm{\gamma}}(E_\mathrm{\alpha})$. Of interest for us is the excitation function for at least one neutron in the decay channel: $\sigma_\mathrm{\alpha,n}(E_\mathrm{\alpha})=\sum_x \sum_y \sigma_{\mathrm{\alpha},x \mathrm{n} y \mathrm{\gamma}}(E_\mathrm{\alpha})$.
%For example, for an \textalpha with a kinetic energy $E_\mathrm{\alpha}=\SI{8}{\MeV}$ incident on \ce{xxx} ($S_\mathrm{\alpha}=\SI{xxx}{\MeV}$ \cite{xxx}, $S_\mathrm{n}=\SI{xxx}{\MeV}$ \cite{xxx}), the emission of up to xxx neutrons is energetical allowed.

In the range of resolved resonances on individual levels, i.e.\ where the width of the peaks in $\sigma_\mathrm{\alpha,n}(E_\mathrm{\alpha})$ is smaller than their spacing, the reaction has to be described by R-matrix theory (see e.g.\ \cite{Descouvemont2010}). Once the spacing drops below the peak's width in the range of unresolved resonances, the reaction can be treated in a statistical way. As the spacing depends on the level density that increases with the mass of the nucleus, the energy below which the statistical treatment breaks down increases with decreasing nuclide mass.

The formation and decay of the compound nucleus can be statistical treated by the  Hauser-Feshbach theory \cite{Hauser1952}. Generally, the exit channels are treated as independent from the entrance channel; remaining correlations between them at low energy are treated by \emph{width fluctuation corrections}. The transmission coefficients for the entrance and exit channels are commonly calculated within an optical model (see e.g.\ \cite{Carlson2001,Capote2009}), i.e.\ describing the elastic scattering and the inelastic scattering via the real and imaginary parts of a complex optical model potential (OMP), respectively. The basic OMPs for spherical nuclides may be generalized for deformed nuclides to coupled-channels (CC) optical models. For weak coupling, the distorted wave-Born approximation (DWBA) can be applied to the CC OMP. Albeit by definition the statistical treatment cannot describe the resolved resonances, it can describe the average behaviour of the relevant physical quantities in this energy range \cite{Rochman2013}: based on these average values and the underlying distributions, it is possible to randomly sample resonances to populate the range of resolved resonances. Albeit the individual resonances created this way depend on the used random seeds, their average behaviour is physical sound.

Concerning the OMPs, they can be broadly divided in two classes \cite{Capote2009}: phenomenological or microscopic OMPs. For both classes, models may include dispersion, i.e.\ do not treat the real and imaginary parts of the complex potential as independent, and hence reducing ambiguities in their parameters. The microscopic OMPs rely on folding the target matter distribution with OMP in nuclear matter, whereas phenomenological OMPs parameterize experimental data, either for an individual nuclide (\emph{local} OMP) or for a larger set of nuclides (\emph{global} OMP). Global phenomenological OMPs are optimized in such a way that, on average, they reproduce cross-sections close to the experimental ones for all non-actinide nuclides. This means there are some nuclides, for example, \ce{^13C}, for which the calculated numbers are not very reliable and extra tuning or even changing to a dedicated local OMP is desirable. For a discussion of suitable OMPs, see section~\ref{sec:Uncertainty:model}.

Nuclear reaction codes that implement the relevant models, and which are widely used and actively maintained are TALYS and EMPIRE. Both use for OMP calculation external tools: TALYS rely on ECIS-06\footnote{Available at \url{https://www-nds.iaea.org/RIPL-3/codes/ECIS/}.} \cite{Raynal1972}; also EMPIRE can use ECIS-06 but offer alternatively OPTMAN in the unpublished version 12\footnote{The older version 10 is available at \url{https://www-nds.iaea.org/RIPL-3/codes/OPTMAN/}.} \cite{Soukhovitskil2008} which has an improved treatment of rotational levels for CC calculations. As both TALYS and EMPIRE are based on similar statistical models, their results are not significantly different from each other. Comprehensive comparison between the two codes, TALYS and EMPIRE, and experimental data for a number of key nuclides has been reported in Ref.~\cite{zakhary,kudryavtsev_neutron_2020}.

%Two approaches with different modifications are applied for \alphan\ cross sections calculations. The first one is the optical model and the second is the compound nucleus model. Usually, the cross sections are first calculated using an optical model, and if the results are not unsatisfactory in comparison with experimental data, then the compound nucleus model is applied.

%Considering the optical model, the computed cross sections can significantly vary for different optical potentials. The codes like TALYS~\cite{talys} are optimized in such a way that, on average, they reproduce cross-sections close to the experimental ones for all non-actinide nuclei. This means there are some nuclides, for example, \ce{^13C}, for which the calculated numbers are not very reliable and extra tuning or even changing of the optical potential is desirable. The modern standard potentials are the options proposed by Koning and Delaroche \cite{Koning:2003zz} and Avrigeanu \it{et al.}\cite{Avrigeanu:2014hma}.

%Another commonly used code for calculating cross-sections is EMPIRE~\cite{empire}. It is based on similar statistical models as TALYS with results not significantly different from the TALYS ones. Comprehensive comparison between the two codes, TALYS and EMPIRE, and experimental data for a number of key isotopes has been reported in Ref.~\cite{zakhary,kudryavtsev_neutron_2020}. 

{\color{red} MP: 

For $^{40}$Ar($\alpha$,n)$^{43}$Ca there is one experimental value available at E$_{\alpha}$=7.4 MeV
(doi:10.1103/PhysRev.101.1370)

For $^{42}$Ca($\alpha$,n)$^{45}$Ti there are experimental cross sections available for E$_{\alpha}$ between 5.7 MeV and 12 MeV
(doi:10.1088/0305-4616/5/9/010)

For $^{116}$Cd($\alpha$,n)$^{50}$Sn$^m$ there are 2 experimental cross sections available for E$_{\alpha}$= 6.18 MeV and 7 MeV (doi:10.1016/0022-1902(81)80372-7)

In Introduction the XENON experiment is mentioned. Should Xe* be added to this table? - no data available in EXFOR in the 4-10 MeV energy range.
}




